Small Parsimony for Natural Genomes in the DCJ-Indel Model

Reconstructing ancestral gene orders is an important step towards understanding genome evolution. The Small Parsimony Problem (SPP) has been extensively studied in this regard. The problem aims at finding the gene orders at internal nodes of a given phylogenetic tree such that the overall genome rearrangement distance along the tree branches is minimized. However, this problem is intractable in most genome rearrangement models, especially when gene duplication and loss are considered. In this work, we describe an Integer Linear Program algorithm to solve the SPP for natural genomes, i.e., genomes that contain conserved, unique, and duplicated markers. The evolutionary model that we consider is the DCJ-indel model that includes the Double-Cut and Join rearrangement operation and the insertion and deletion of genome segments. We evaluate our algorithm on simulated data and show that it is able to reconstruct very efficiently and accurately ancestral gene orders in a very comprehensive evolutionary model.

==> main-diagrams.tex <==
\begin{tikzpicture}[/tikzinclude/figure=speciestree, scale=0.5,
        every node/.style={transform shape, fill, circle, minimum
    height=2pt,minimum width=2pt,inner sep=0, outer sep=1pt}]

    \node[label=above:$E$](e) {};
    \node[label=left:$D$](d) at ($(e) + (-0.5, -0.5cm)$) {};
    \node[label=below:$A$](a) at ($(d) + (-0.5, -1.2cm)$) {};
    \node[label=below:$B$](b) at ($(d) + (0.5, -1.2cm)$) {};
    \node[label=below:$C$](c) at ($(e) + (0.75, -1.7cm)$) {};
    \draw (a) -- (d) -- (e) -- (c);
    \draw (d) -- (b);

\end{tikzpicture}

\begin{tikzpicture}[/tikzinclude/figure=genetree1, scale=0.6,
        every node/.style={transform shape, fill, circle, minimum
        height=2pt,minimum width=2pt,inner sep=0, outer sep=1pt}]

    \node[label={[label distance=-2ex]90:$4.1_E$}](e4) {};
    \node[label=left:$4.1_D$](d4) at ($(e4) + (-0.75, -0.3cm)$) {};
    \node[label={[label distance=-2ex]270:$4.1_A$}](a4) at ($(d4) + (-0.5, -1.4cm)$) {};
    \node[label={[label distance=-1ex]180:$4.2_B$}](b41) at ($(d4) + (0.5, -0.5cm)$) {};
    \node[label={[label distance=-2ex]270:$4.1_B$}](b42) at ($(b41) + (-0.3, -0.9cm)$) {};
    \node[fill=none] (b43) at ($(b41) + (0.3, -0.9cm)$) {\tiny\faClose};
    \node[label={[label distance=-2ex]270:$4.1_C$}](c43) at ($(e4) + (0.75, -1.7cm)$) {};
    \draw (a4) -- (d4) -- (e4) -- (c43);
    \draw (d4) -- (b41) -- (b42);
    \draw (b41) -- (b43);
\end{tikzpicture}

\begin{tikzpicture}[/tikzinclude/figure=genetree2, scale=0.6,
        every node/.style={transform shape, fill, circle, minimum
        height=2pt,minimum width=2pt,inner sep=0, outer sep=1pt}]

    \node[label={[label distance=-2ex]90:$2.1_E$}](e2) {};
    \node[label=left:$2.1_D$](d2) at ($(e2) + (-0.75, -0.3cm)$) {};
    \node[fill=none] (a2) at ($(d2) + (-0.5, -1.4cm)$) {\tiny\faClose};
    \node[label={[label distance=-1ex]180:$2.3_B$}](b21) at ($(d2) + (0.5, -0.5cm)$) {};
    \node[label={[label distance=-2ex]270:$2.1_B$}](b22) at ($(b21) + (-0.35, -0.9cm)$) {};
    \node[label={[label distance=-2ex]270:$2.2_B$}](b23) at ($(b21) + (0.35, -0.9cm)$) {};
    \node[label=right:$2.3_C$](c21) at ($(e2) + (1.2, -0.8cm)$) {};
    \node[label={[label distance=-2ex]270:$2.1_C$}](c22) at ($(c21) + (-0.35, -0.9cm)$) {};
    \node[label={[label distance=-2ex]270:$2.2_C$}](c23) at ($(c21) + (0.35, -0.9cm)$) {};
    \draw (a2) -- (d2) -- (e2) -- (c21) -- (c22);
    \draw (d2) -- (b21) -- (b22);
    \draw (b21) -- (b23);
    \draw (c21) -- (c23);
\end{tikzpicture}

\begin{tikzpicture}[/tikzinclude/figure=reconciledtrees, scale=0.6,
        every node/.style={transform shape, fill, circle, minimum
        height=2pt,minimum width=2pt,inner sep=0, outer sep=1pt}]

    \node[label={[label distance=-2ex]90:$4.1_E$}](e4) {};
    \node[label=left:$4.1_D$](d4) at ($(e4) + (-0.75, -0.3cm)$) {};
    \node[label={[label distance=-2ex]270:$4.1_A$}](a4) at ($(d4) + (-0.5, -1.4cm)$) {};
    \node[label={[label distance=-1ex]180:$4.2_B$}](b41) at ($(d4) + (0.5, -0.5cm)$) {};
    \node[label={[label distance=-2ex]270:$4.1_B$}](b42) at ($(b41) + (-0.3, -0.9cm)$) {};
    \node[fill=none] (b43) at ($(b41) + (0.3, -0.9cm)$) {\tiny\faClose};
    \node[label={[label distance=-2ex]270:$4.1_C$}](c43) at ($(e4) + (0.75, -1.7cm)$) {};
    \draw (a4) -- (d4) -- (e4) -- (c43);
    \draw (d4) -- (b41) -- (b42);
    \draw (b41) -- (b43);

    \node[right=3cm of e4,label={[label distance=-2ex]90:$2.1_E$}](e2) {};
    \node[label=left:$2.1_D$](d2) at ($(e2) + (-0.75, -0.3cm)$) {};
    \node[fill=none] (a2) at ($(d2) + (-0.5, -1.4cm)$) {\tiny\faClose};
    \node[label={[label distance=-1ex]180:$2.3_B$}](b21) at ($(d2) + (0.5, -0.5cm)$) {};
    \node[label={[label distance=-2ex]270:$2.1_B$}](b22) at ($(b21) + (-0.35, -0.9cm)$) {};
    \node[label={[label distance=-2ex]270:$2.2_B$}](b23) at ($(b21) + (0.35, -0.9cm)$) {};
    \node[label=right:$2.3_C$](c21) at ($(e2) + (1.2, -0.8cm)$) {};
    \node[label={[label distance=-2ex]270:$2.1_C$}](c22) at ($(c21) + (-0.35, -0.9cm)$) {};
    \node[label={[label distance=-2ex]270:$2.2_C$}](c23) at ($(c21) + (0.35, -0.9cm)$) {};
    \draw (a2) -- (d2) -- (e2) -- (c21) -- (c22);
    \draw (d2) -- (b21) -- (b22);
    \draw (b21) -- (b23);
    \draw (c21) -- (c23);
    \draw[densely dotted,color=red!80!black] (e2) to[out=160, in=20] (e4);
    \draw[densely dotted,color=red!80!black] (d2) to[out=160, in=20] (d4);
    \draw[densely dotted,color=red!80!black] (b21) to[out=160, in=20] (b41);
    \draw[densely dotted,color=red!80!black] (c21) to[out=200, in=40] (c43);

\end{tikzpicture}

\begin{tikzpicture}[/tikzinclude/figure=adjforest, scale=0.6,
        every node/.style={transform shape, fill, circle, minimum
        height=2pt,minimum width=2pt,inner sep=0, outer sep=1pt}]

    \clip (-2.5,0.41) rectangle + (5.4,-3);
    \node[label={[label distance=-6.5ex]90:$\{4.1_E^\eh, 2.1_E^\et\}$}](e2) {};
    \node[label=left:{$\{4.1_D^\eh,2.1_D^\et\}$}](d2) at ($(e2) + (-0.75, -0.3cm)$) {};
    \node[fill=none] (a2) at ($(d2) + (-0.5, -1.4cm)$) {\tiny\faClose};
    \node[](b21) at ($(d2) + (0.5, -0.5cm)$) {};
    \node[fill=none,right=-1ex of b21,text width=12ex]{$\{4.2_B^\eh,$
    \phantom{bl}$2.3_B^\et\}$};
    \node[label={[label distance=-6ex]270:$\{4.1_B^\eh, 2.1_B^\et\}$}](b22) at ($(b21) + (-0.35, -0.9cm)$) {};
    \node[fill=none] (b23) at ($(b21) + (0.35, -0.9cm)$) {\tiny\faClose};
    \node[label=right:{$\{4.1_C^\eh, 2.3_C^\et\}$}](c21) at ($(e2) + (1.2, -0.8cm)$) {};
    \node[label={[label distance=-6ex]270:$\{4.1_C^\eh, 2.2_C^\et\}$}](c23) at ($(c21) + (0.35, -0.9cm)$) {};
    \draw (a2) -- (d2) -- (e2) -- (c21) -- (c23);
    \draw (d2) -- (b21) -- (b22);
    \draw (b21) -- (b23);
\end{tikzpicture}


\begin{tikzpicture}[/tikzinclude/figure=degenerate_genomes, every
    node/.style={fill, circle, minimum height=2pt,minimum width=2pt,inner
    sep=0, outer sep=2pt}, elabel/.style={midway,fill=white,fill opacity=0.8,
    text=black!60,font=\tiny}]

    \node[label=above:$1_A^\et$](1at) {};
    \node[right=1cm of 1at,label=above:$1_A^\eh$] (1ah) {};
    \node[below=1cm of 1at,label=below:$2_A^\et$] (2at) {};
    \node[right=1cm of 2at,label=below:$2_A^\eh$] (2ah) {};

    \draw (1at) -- (2at);
    \draw (1ah) -- (2ah);
    \draw[dotted] (1at) -- (1ah);
    \draw[dotted] (2at) -- (2ah);

%        \node[right=1.7cm of 2bh,label=below:$t.1_C^\circ$] (t3ch) {};
%        \node[right=1cm of t3ch,label=below:$3_C^\eh$] (3ch) {};
%        \node[above=1cm of 3ch,label=above:$2_C^\et$] (2ct) {};
%        \node[right=1cm of 2ct,label=above:$2_C^\eh$] (2ch) {};
%        \node[right=1cm of 3ch,label=below:$3_C^\et$] (3ct) {};
%        \node[right=1cm of 2ch,label=above:$1_C^\et$] (1ct) {};
%        \node[below=1cm of 1ct,label=below:$1_C^\eh$] (1ch) {};
%        \draw (1ct) to[out=0,in=0] (1ch);
%        \draw (2ch) -- (3ct);
%        \draw (2ct) -- (3ct);
%        \draw (3ch) -- (t3ch);
%        \draw[dotted] (1ct) -- (1ch);
%        \draw[dotted] (2ct) -- (2ch);
%        \draw[dotted] (3ct) -- (3ch);

    \node[right=3cm of 1ah,label={[yshift=-2pt]$1_B^\et$}] (1ct) {};
    \node[right=0.5cm of 1ct,label={[yshift=-3pt]$2_B^\et$}] (2ct) {};
    \node[position=-60:0.5cm from 1ct,label={[xshift=10pt,yshift=-12pt]$3_B^\et$}] (3ct) {};
    \node[position=150:1cm from 1ct,label=left:$1_B^\eh$] (1ch) {};
    \node[position=30:1cm from 2ct,label=right:$2_B^\eh$] (2ch) {};
    \node[position=-90:1cm from 3ct,label=right:$3_B^\eh$] (3ch) {};

    \draw (1ct) -- (2ct) -- (3ct) -- (1ct);
    \draw (1ch) -- (2ch) -- (3ch) -- (1ch);
    \draw[dotted] (1ct) -- (1ch);
    \draw[dotted] (2ct) -- (2ch);
    \draw[dotted] (3ct) -- (3ch);
    
    \node[right=3cm of 2ct,label=above:$1_C^\et$] (1bt) {};
    \node[right=1cm of 1bt,label=above:$1_C^\eh$] (1bh) {};
    \node[below=1cm of 1bt,label=below:$2_C^\et$] (2bt) {};
    \node[right=1cm of 2bt,label=below:$2_C^\eh$] (2bh) {};
    \node[right=1cm of 1bh,label=above:$t.2_C^\circ$] (t1bh) {};
    \node[right=1cm of 2bh,label=below:$t.3_C^\circ$] (t2bh) {};
    \node[left=1cm of 2bt,label=below:$t.1_C^\circ$] (t2bt) {};

    \draw (1bt) -- (2bt);
    \draw (1bh) -- (2bh);
    \draw (1bt) -- (2bh);
    \draw (1bh) -- (2bt);
    \draw (1bh) -- (t1bh);
    \draw (2bh) -- (t2bh);
    \draw (2bt) -- (t2bt);
    \draw[dotted] (1bt) -- (1bh);
    \draw[dotted] (2bt) -- (2bh);


    \node[fill=none,font=\boldmath\large] at ($(2at.east) + (0.5, -1.1)$) {$A$};
    \node[fill=none,font=\boldmath\large] at ($(2bh) + (0, -1.1)$) {$C$};
    \node[fill=none,font=\boldmath\large] at ($(3ch.east) + (0, -0.5)$) {$B$};

\end{tikzpicture}


\begin{tikzpicture}[/tikzinclude/figure=relational_diagram, scale=0.44,
    every node/.style={transform shape, fill, circle, minimum
    height=4pt,minimum width=4pt,inner sep=0, outer sep=3pt,font=\Large},
    every path/.style={line width=0.8},
    dots/.style={line cap=round, line width=0.8, dash pattern=on 0pt off 2},
    tel/.style={fill=none,draw}, 
    mrd/.style={color=black!40,},
    mrdd/.style={color=black!10,line width=0.4},
    a/.style={color=magenta}, b/.style={color=green!70!black}]%!30!yellow}]

    \coordinate (v0);
    \node[tel,b,right=1.2cm of v0, label=above:{$t.1_A^\circ$}](v1) {};
    \node[b,label=above:{$1_A^\et$},right=1cm of v1](v2) {};
    \node[label=above:{$1_A^\eh$},right=1cm of v2](v3) {};
    \node[label=above:{$2_A^\eh$},right=1cm of v3](v4) {};
    \node[b,label=above:{$2_A^\et$},right=1cm of v4](v5) {};
    \node[a,label=above:{$3_A^\eh$},right=1cm of v5](v6) {};
    \node[a,label=above:{$3_A^\et$},right=1cm of v6](v7) {};
    \node[a,tel,label=above:{$t.2_A^\circ$},right=1cm of v7](v8) {};
    \node[tel,label=above:{$t.3_A^\circ$},right=1cm of v8](v9) {};
    \node[label=above:{$4_A^\et$},right=1cm of v9](v10) {};
    \node[label=above:{$4_A^\eh$},right=1cm of v10](v11) {};
    \node[label=above:{$5_A^\et$},right=1cm of v11](v12) {};
    \node[label=above:{$5_A^\eh$},right=1cm of v12](v13) {};
    \node[tel,label=above:{$t.4_A^\circ$},right=1cm of v13](v14) {};
    \node[tel,label=above:{$t.5_A^\circ$},right=1cm of v14](v15) {};
    \node[label=above:{$6_A^\et$},right=1cm of v15](v16) {};
    \node[b,label=above:{$6_A^\eh$},right=1cm of v16](v17) {};
    \node[a,label=above:{$7_A^\eh$},right=1cm of v17](v18) {};
    \node[a,label=above:{$7_A^\et$},right=1cm of v18](v19) {};
    \node[a,label=above:{$8_A^\et$},right=1cm of v19](v20) {};
    \node[label=above:{$8_A^\eh$},right=1cm of v20](v21) {};
    \node[tel,label=above:{$t.6_A^\circ$},right=1cm of v21](v22) {};

    \node[tel,label=below:{$t.1_B^\circ$},below=4cm of v0](v41) {};
    \node[label=below:{$1_B^\eh$},right=1cm of v41](v42) {};
    \node[b,label=below:{$1_B^\et$},right=1cm of v42](v43) {};
    \node[b,label=below:{$9_B^\et$},right=1cm of v43](v44) {};
    \node[b,label=below:{$9_B^\eh$},right=1cm of v44](v45) {};
    \node[b,label=below:{$2_B^\et$},right=1cm of v45](v46) {};
    \node[label=below:{$2_B^\eh$},right=1cm of v46](v47) {};
    \node[label=below:{$4_B^\et$},right=1cm of v47](v48) {};
    \node[label=below:{$4_B^\eh$},right=1cm of v48](v49) {};
    \node[label=below:{$5_B^\et$},right=1cm of v49](v50) {};
    \node[label=below:{$5_B^\eh$},right=1cm of v50](v51) {};
    \node[tel,label=below:{$t.2_B^\circ$},right=1cm of v51](v52) {};
    \node[tel,mrd,label={[label distance=-1.39cm,mrd]:$t.3_B^\circ$},right=1cm of v52](v63) {};
    \node[tel,mrd,label={[label distance=-1.39cm,mrd]:$t.4_B^\circ$},right=1cm of v63](v64) {};
    \node[b,label=below:{$10_B^\et$},right=1cm of v64](v61) {};
    \node[b,label=below:{$10_B^\eh$},right=1cm of v61](v62) {};
    \node[tel,a,label=below:{$t.5_B^\circ$},right=1cm of v62](v53) {};
    \node[a,label=below:{$8_B^\et$},right=1cm of v53](v54) {};
    \node[label=below:{$8_B^\eh$},right=1cm of v54](v55) {};
    \node[label=below:{$6_B^\et$},right=1cm of v55](v56) {};
    \node[b,label=below:{$6_B^\eh$},right=1cm of v56](v57) {};
    \node[b,label=below:{$11_B^\eh$},right=1cm of v57](v58) {};
    \node[b,label=below:{$11_B^\et$},right=1cm of v58](v59) {};
    \node[b,tel,label=below:{$t.6_B^\circ$},right=1cm of v59](v60) {};

    
    \draw[b] (v1) -- (v2);
    \draw (v3) -- (v4);
    \draw[bicolor={b}{a}] (v5) -- (v6);
    \draw[a] (v7) -- (v8);
    \draw (v9) -- (v10);
    \draw (v11) -- (v12);
    \draw (v13) -- (v14);
    \draw (v15) -- (v16);
    \draw[bicolor={b}{a}] (v17) -- (v18);
    \draw[a] (v19) -- (v20);
    \draw (v21) -- (v22);

    \draw (v41) -- (v42);
    \draw[b] (v43) -- (v44);
    \draw[b] (v45) -- (v46);
    \draw (v47) -- (v48);
    \draw (v49) -- (v50);
    \draw (v51) -- (v52);
    \draw[a] (v53) -- (v54);
    \draw (v55) -- (v56);
    \draw[b] (v57) -- (v58);
    \draw[b] (v59) -- (v60);
    \draw[b] (v61) -- (v62);
    \draw[mrd] (v63) -- (v64);


    \draw[a,dots] (v6) -- (v7);
    \draw[a,dots] (v18) -- (v19);
    \draw[b,dots] (v44) -- (v45);
    \draw[b,dots] (v58) -- (v59);
    \draw[b,dots] (v61) to[out=90, in=90] (v62);

    \draw[mrdd,dashed] (v1) -- (v60);
    \draw[mrdd,dashed] (v1) -- (v53);
    \draw[mrdd,dashed] (v1) -- (v41);
    \draw[mrdd,dashed] (v1) -- (v52);
    \draw[mrdd,dashed] (v1) -- (v63);
    \draw[mrdd,dashed] (v1) -- (v64);

    \draw[mrdd,dashed] (v8) -- (v60);
    \draw[mrdd,dashed] (v8) -- (v53);
    \draw[mrdd,dashed] (v8) -- (v41);
    \draw[mrdd,dashed] (v8) -- (v52);
    \draw[mrdd,dashed] (v8) -- (v63);
    \draw[mrdd,dashed] (v8) -- (v64);

    \draw[mrdd,dashed] (v9) -- (v60);
    \draw[mrdd,dashed] (v9) -- (v53);
    \draw[mrdd,dashed] (v9) -- (v41);
    \draw[mrdd,dashed] (v9) -- (v52);
    \draw[mrdd,dashed] (v9) -- (v63);
    \draw[mrdd,dashed] (v9) -- (v64);

    \draw[mrdd,dashed] (v14) -- (v60);
    \draw[mrdd,dashed] (v14) -- (v53);
    \draw[mrdd,dashed] (v14) -- (v41);
    \draw[mrdd,dashed] (v14) -- (v52);
    \draw[mrdd,dashed] (v14) -- (v63);
    \draw[mrdd,dashed] (v14) -- (v64);

    \draw[mrdd,dashed] (v15) -- (v60);
    \draw[mrdd,dashed] (v15) -- (v53);
    \draw[mrdd,dashed] (v15) -- (v41);
    \draw[mrdd,dashed] (v15) -- (v52);
    \draw[mrdd,dashed] (v15) -- (v63);
    \draw[mrdd,dashed] (v15) -- (v64);

    \draw[mrdd,dashed] (v22) -- (v60);
    \draw[mrdd,dashed] (v22) -- (v53);
    \draw[mrdd,dashed] (v22) -- (v41);
    \draw[mrdd,dashed] (v22) -- (v52);
    \draw[mrdd,dashed] (v22) -- (v63);
    \draw[mrdd,dashed] (v22) -- (v64);

    \draw[mrd,dashed] (v1) -- (v60);
    \draw[mrd,dashed] (v8) -- (v53);
    \draw[mrd,dashed] (v9) -- (v41);
    \draw[mrd,dashed] (v14) -- (v52);
    \draw[mrd,dashed] (v15) -- (v63);
    \draw[mrd,dashed] (v22) -- (v64);
    

    \draw[b,dashed] (v2) -- (v43);
    \draw[dashed] (v3) -- (v42);
    \draw[dashed] (v4) -- (v47);
    \draw[b,dashed] (v5) -- (v46);
    \draw[dashed] (v10) -- (v48);
    \draw[dashed] (v11) -- (v49);
    \draw[dashed] (v12) -- (v50);
    \draw[dashed] (v13) -- (v51);
    \draw[dashed] (v16) -- (v56);
    \draw[b,dashed] (v17) -- (v57);
    \draw[a,dashed] (v20) -- (v54);
    \draw[dashed] (v21) -- (v55);


\end{tikzpicture}

